On the Decay of Sunspot Groups and Their Internal Parts in Detail

The decay of sunspot groups is a relatively unknown field since most studies have focused mainly on the decay of sunspots or sunspot groups, but only on small samples. As an extension of the recent work of \citet{2020ApJ...892..107M} which is based on a large verified sample, this study investigates not only the long-term behavior of the decay of sunspot groups but also the dynamics of their parts. The aim of the present work is to search for dependencies of the decay process in order to find physical conditions that modify or contribute to the decay. The investigations are based on the catalog of SoHO Debrecen Sunspot Database (SDD ) and the Greenwich Photoheliographic Results (GPR) as well as the Debrecen Photoheliographic Data (DPD). Altogether more than 750 sunspot groups were considered. The decay rates have been calculated for the total, umbral and penumbral area of the groups and in the case of the SDD's groups they have been calculated for both the leading and the following parts. The decay rates depend linearly on the maximum areas and ranged from 30-50 MSH/day for the sunspot groups and penumbrae and 5-10 MSH/day for the umbrae throughout the cycle. The decay rates fall significantly during the Gnevyshev gap and show 4+4 Schwabe cyclical variations in the ascending/descending phases, but it is always higher in the northern hemisphere. There is a slight decrease of the decay rates in the activity range toward higher latitudes.

==> Murakozy_biblio <==
@ARTICLE{2016SoPh..291.3081B,
       author = {{Baranyi}, T. and {Gy{\H{o}}ri}, L. and {Ludm{\'a}ny}, A.},
        title = "{On-line Tools for Solar Data Compiled at the Debrecen Observatory and Their Extensions with the Greenwich Sunspot Data}",
      journal = {\solphys},
     keywords = {Sunspots, Active regions, Magnetic fields, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = nov,
       volume = {291},
       number = {9-10},
        pages = {3081-3102},
          doi = {10.1007/s11207-016-0930-1},
archivePrefix = {arXiv},
       eprint = {1606.00669},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016SoPh..291.3081B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015MNRAS.447.1857B,
       author = {{Baranyi}, T.},
        title = "{Comparison of Debrecen and Mount Wilson/Kodaikanal sunspot group tilt angles and the Joy's law}",
      journal = {\mnras},
     keywords = {methods: data analysis, sunspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = feb,
       volume = {447},
       number = {2},
        pages = {1857-1865},
          doi = {10.1093/mnras/stu2572},
archivePrefix = {arXiv},
       eprint = {1412.1355},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.447.1857B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020ApJ...892..107M,
       author = {{Murak{\"o}zy}, Judit},
        title = "{Study of the Decay Rates of the Umbral Area of Sunspot Groups Using a High-resolution Database}",
      journal = {\apj},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = apr,
       volume = {892},
       number = {2},
          eid = {107},
        pages = {107},
          doi = {10.3847/1538-4357/ab7898},
archivePrefix = {arXiv},
       eprint = {2002.08997},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...892..107M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019NCimC..42...11M,
       author = {{Murabito}, M. and {Romano}, P. and {Zuccarello}, F. and
         {Guglielmino}, S.~L.},
        title = "{Recent insights on the penumbra formation process}",
      journal = {Nuovo Cimento C Geophysics Space Physics C},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = jan,
       volume = {42},
       number = {1},
          eid = {11},
        pages = {11},
          doi = {10.1393/ncc/i2019-19011-4},
archivePrefix = {arXiv},
       eprint = {1901.05207},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019NCimC..42...11M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017ApJ...834...76M,
       author = {{Murabito}, M. and {Romano}, P. and {Guglielmino}, S.~L. and
         {Zuccarello}, F.},
        title = "{On the Formation of a Stable Penumbra in a Region of Flux Emergence in the Sun}",
      journal = {\apj},
     keywords = {Sun: chromosphere, Sun: magnetic fields, Sun: photosphere, sunspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jan,
       volume = {834},
       number = {1},
          eid = {76},
        pages = {76},
          doi = {10.3847/1538-4357/834/1/76},
archivePrefix = {arXiv},
       eprint = {1611.04749},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...834...76M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014PASJ...66S..11K,
       author = {{Kitai}, Reizaburo and {Watanabe}, Hiroko and {Otsuji}, Ken'ichi},
        title = "{Morphological study of penumbral formation}",
      journal = {\pasj},
     keywords = {convection, Sun: magnetic fields, Sun: photosphere, sunspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = dec,
       volume = {66},
          eid = {S11},
        pages = {S11},
          doi = {10.1093/pasj/psu084},
archivePrefix = {arXiv},
       eprint = {1407.4573},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014PASJ...66S..11K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...784...10R,
       author = {{Romano}, P. and {Guglielmino}, S.~L. and {Cristaldi}, A. and
         {Ermolli}, I. and {Falco}, M. and {Zuccarello}, F.},
        title = "{Evolution of the Magnetic Field Inclination in a Forming Penumbra}",
      journal = {\apj},
     keywords = {Sun: chromosphere, Sun: magnetic fields, Sun: photosphere},
         year = 2014,
        month = mar,
       volume = {784},
       number = {1},
          eid = {10},
        pages = {10},
          doi = {10.1088/0004-637X/784/1/10},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...784...10R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013SoPh..286..347H,
       author = {{Hathaway}, D.~H.},
        title = "{A Curious History of Sunspot Penumbrae}",
      journal = {\solphys},
     keywords = {Active regions, structure, Sunspots, penumbra, statistics, umbra, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = sep,
       volume = {286},
       number = {2},
        pages = {347-356},
          doi = {10.1007/s11207-013-0291-y},
archivePrefix = {arXiv},
       eprint = {1304.8060},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013SoPh..286..347H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013MmSAI..84..428G,
       author = {{Gafeira}, R. and {Fonte}, C.~C. and {Pais}, M.~A. and {Fernandes}, J.},
        title = "{Variation rate of sunspot area}",
      journal = {\memsai},
     keywords = {Sun: Sunspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = jan,
       volume = {84},
        pages = {428},
archivePrefix = {arXiv},
       eprint = {1211.6870},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MmSAI..84..428G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2012ASPC..455...61S,
       author = {{Schlichenmaier}, R. and {Rezaei}, R. and {Gonz{\'a}lez}, N.~B.},
        title = "{On the Formation of Penumbrae as Observed with the German VTT SOHO/MDI, and SDO/HMI}",
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
    booktitle = {4th Hinode Science Meeting: Unsolved Problems and Recent Insights},
         year = 2012,
       editor = {{Bellot Rubio}, L. and {Reale}, F. and {Carlsson}, M.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {455},
        month = may,
        pages = {61},
archivePrefix = {arXiv},
       eprint = {1102.0965},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ASPC..455...61S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...538A.109V,
       author = {{Verma}, M. and {Balthasar}, H. and {Deng}, N. and {Liu}, C. and
         {Shimizu}, T. and {Wang}, H. and {Denker}, C.},
        title = "{Horizontal flow fields observed in Hinode G-band images. II. Flow fields in the final stages of sunspot decay}",
      journal = {\aap},
     keywords = {methods: data analysis, Sun: chromosphere, Sun: photosphere, Sun: surface magnetism, sunspots, techniques: image processing, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = feb,
       volume = {538},
          eid = {A109},
        pages = {A109},
          doi = {10.1051/0004-6361/201117842},
archivePrefix = {arXiv},
       eprint = {1112.1589},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...538A.109V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2011AGUFMSH52B..02R,
       author = {{Rempel}, M. and {Cheung}, M. and {Birch}, A.~C. and {Braun}, D.~C.},
        title = "{Numerical simulations of the subsurface structure of sunspots}",
     keywords = {7522 SOLAR PHYSICS, ASTROPHYSICS, AND ASTRONOMY / Helioseismology, 7524 SOLAR PHYSICS, ASTROPHYSICS, AND ASTRONOMY / Magnetic fields, 7529 SOLAR PHYSICS, ASTROPHYSICS, AND ASTRONOMY / Photosphere},
    booktitle = {AGU Fall Meeting Abstracts},
         year = 2011,
       volume = {2011},
        month = dec,
          eid = {SH52B-02},
        pages = {SH52B-02},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011AGUFMSH52B..02R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...671.1013D,
       author = {{Deng}, Na and {Choudhary}, Debi Prasad and {Tritschler}, Alexandra and
         {Denker}, Carsten and {Liu}, Chang and {Wang}, Haimin},
        title = "{Flow Field Evolution of a Decaying Sunspot}",
      journal = {\apj},
     keywords = {Instrumentation: High Angular Resolution, Instrumentation: Spectrographs, Sun: Activity, Sun: Photosphere, Sun: Sunspots, Techniques: Spectroscopic, Astrophysics},
         year = 2007,
        month = dec,
       volume = {671},
       number = {1},
        pages = {1013-1021},
          doi = {10.1086/523102},
archivePrefix = {arXiv},
       eprint = {0709.3340},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...671.1013D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1976Ap&SS..40...73P,
       author = {{Piddington}, J.~H.},
        title = "{Solar Magnetic Fields and Convection. IV: Magnetic Flux Ropes and Their Fibres}",
      journal = {\apss},
     keywords = {Lines Of Force, Magnetic Field Configurations, Magnetic Flux, Solar Magnetic Field, Dynamo Theory, Magnetic Effects, Stellar Models, Sunspots, Solar Physics},
         year = 1976,
        month = mar,
       volume = {40},
       number = {1},
        pages = {73-90},
          doi = {10.1007/BF00651189},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1976Ap&SS..40...73P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018ApJ...865...88C,
       author = {{Carrasco}, V.~M.~S. and {Garc{\'\i}a-Romero}, J.~M. and
         {Vaquero}, J.~M. and {Rodr{\'\i}guez}, P.~G. and {Foukal}, P. and
         {Gallego}, M.~C. and {Lef{\`e}vre}, L.},
        title = "{The Umbra-Penumbra Area Ratio of Sunspots During the Maunder Minimum}",
      journal = {\apj},
     keywords = {Sun: activity, Sun: general, sunspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = oct,
       volume = {865},
       number = {2},
          eid = {88},
        pages = {88},
          doi = {10.3847/1538-4357/aad9f6},
archivePrefix = {arXiv},
       eprint = {1809.08670},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...865...88C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008SoPh..250..269H,
       author = {{Hathaway}, David H. and {Choudhary}, Debi Prasad},
        title = "{Sunspot Group Decay}",
      journal = {\solphys},
     keywords = {Sun: sunspots, Sun: active regions},
         year = 2008,
        month = aug,
       volume = {250},
       number = {2},
        pages = {269-278},
          doi = {10.1007/s11207-008-9226-4},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008SoPh..250..269H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1963BAICz..14...91B,
       author = {{Bumba}, V.},
        title = "{Development of SPOT group areas in dependence on the local magnetic field}",
      journal = {Bulletin of the Astronomical Institutes of Czechoslovakia},
         year = 1963,
        month = jan,
       volume = {14},
        pages = {91},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1963BAICz..14...91B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011SoPh..270..463J,
       author = {{Javaraiah}, J.},
        title = "{Long-Term Variations in the Growth and Decay Rates of Sunspot Groups}",
      journal = {\solphys},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = jun,
       volume = {270},
       number = {2},
        pages = {463-483},
          doi = {10.1007/s11207-011-9768-8},
archivePrefix = {arXiv},
       eprint = {1105.1066},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011SoPh..270..463J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992SoPh..137...51H,
       author = {{Howard}, Robert F.},
        title = "{The Growth and Decay of Sunspot Groups}",
      journal = {\solphys},
     keywords = {Solar Atmosphere, Solar Magnetic Field, Sunspots, Umbras, Faculae, Magnetic Field Configurations, Magnetic Flux, Meridional Flow, Solar Rotation, Solar Physics},
         year = 1992,
        month = jan,
       volume = {137},
       number = {1},
        pages = {51-65},
          doi = {10.1007/BF00146575},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992SoPh..137...51H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992SoPh..142...47H,
       author = {{Howard}, Robert F.},
        title = "{Some Characteristics of the Development and Decay of Active Region Magnetic Flux}",
      journal = {\solphys},
     keywords = {Faculae, Solar Magnetic Field, Sunspots, Magnetic Signatures, Solar Rotation, Solar Physics},
         year = 1992,
        month = nov,
       volume = {142},
       number = {1},
        pages = {47-65},
          doi = {10.1007/BF00156633},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992SoPh..142...47H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993A&A...274..521M,
       author = {{Martinez Pillet}, V. and {Moreno-Insertis}, F. and {Vazquez}, M.},
        title = "{The distribution of sunspot decay rates.}",
      journal = {\aap},
     keywords = {sun: activity, sun: photosphere, sun: sunspots},
         year = 1993,
        month = jul,
       volume = {274},
        pages = {521-533},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993A&A...274..521M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995SoPh..157..389L,
       author = {{Lustig}, G. and {Wohl}, H.},
        title = "{The Growth and Decay of Sunspots: Comparison between the Greenwich and Mount Wilson Sunspot Data}",
      journal = {\solphys},
     keywords = {Decay, Growth, Solar Physics, Sun, Sunspots, Latitude, Umbras, Solar Physics},
         year = 1995,
        month = mar,
       volume = {157},
       number = {1-2},
        pages = {389-392},
          doi = {10.1007/BF00680629},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995SoPh..157..389L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002AN....323..342M,
       author = {{Mart{\'\i}nez Pillet}, V.},
        title = "{Decay of sunspots}",
      journal = {Astronomische Nachrichten},
     keywords = {Sun, stars: spots},
         year = 2002,
        month = jul,
       volume = {323},
        pages = {342-348},
          doi = {10.1002/1521-3994(200208)323:3/4<342::AID-ASNA342>3.0.CO;2-5},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002AN....323..342M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020SoPh..295...60H,
       author = {{Hamedivafa}, Hashem},
        title = "{Comparative Study of a Sunspot at Two Different Instances of Time}",
      journal = {\solphys},
     keywords = {Sunspots, umbra, Sunspots, statistics},
         year = 2020,
        month = apr,
       volume = {295},
       number = {4},
          eid = {60},
        pages = {60},
          doi = {10.1007/s11207-020-01627-x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020SoPh..295...60H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019SoPh..294...72J,
       author = {{Jha}, Bibhuti Kumar and {Mandal}, Sudip and {Banerjee}, Dipankar},
        title = "{Study of Sunspot Penumbra to Umbra Area Ratio Using Kodaikanal White-light Digitised Data}",
      journal = {\solphys},
     keywords = {Sunspots, umbra, penumbra, Solar cycle, observations, magnetic fields, statistics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = jun,
       volume = {294},
       number = {6},
          eid = {72},
        pages = {72},
          doi = {10.1007/s11207-019-1462-2},
archivePrefix = {arXiv},
       eprint = {1905.06888},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019SoPh..294...72J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993A&A...274..521M,
       author = {{Martinez Pillet}, V. and {Moreno-Insertis}, F. and {Vazquez}, M.},
        title = "{The distribution of sunspot decay rates.}",
      journal = {\aap},
     keywords = {sun: activity, sun: photosphere, sun: sunspots},
         year = 1993,
        month = jul,
       volume = {274},
        pages = {521-533},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993A&A...274..521M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.419.3624M,
       author = {{Murak{\"o}zy}, J. and {Ludm{\'a}ny}, A.},
        title = "{Phase lags of solar hemispheric cycles}",
      journal = {\mnras},
     keywords = {Sun: activity, Sun: dynamo, sunspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = feb,
       volume = {419},
       number = {4},
        pages = {3624-3630},
          doi = {10.1111/j.1365-2966.2011.20011.x},
archivePrefix = {arXiv},
       eprint = {1309.2114},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.419.3624M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016ApJ...826..145M,
       author = {{Murak{\"o}zy}, J.},
        title = "{Phase Relationships of Solar Hemispheric Toroidal and Poloidal Cycles}",
      journal = {\apj},
     keywords = {Sun: activity, Sun: magnetic fields, sunspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2016,
        month = aug,
       volume = {826},
       number = {2},
          eid = {145},
        pages = {145},
          doi = {10.3847/0004-637X/826/2/145},
archivePrefix = {arXiv},
       eprint = {1605.08230},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...826..145M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002AN....323..342M,
       author = {{Mart{\'\i}nez Pillet}, V.},
        title = "{Decay of sunspots}",
      journal = {Astronomische Nachrichten},
     keywords = {Sun, stars: spots},
         year = 2002,
        month = jul,
       volume = {323},
        pages = {342-348},
          doi = {10.1002/1521-3994(200208)323:3/4<342::AID-ASNA342>3.0.CO;2-5},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002AN....323..342M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017ApJ...834...76M,
       author = {{Murabito}, M. and {Romano}, P. and {Guglielmino}, S.~L. and
         {Zuccarello}, F.},
        title = "{On the Formation of a Stable Penumbra in a Region of Flux Emergence in the Sun}",
      journal = {\apj},
     keywords = {Sun: chromosphere, Sun: magnetic fields, Sun: photosphere, sunspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jan,
       volume = {834},
       number = {1},
          eid = {76},
        pages = {76},
          doi = {10.3847/1538-4357/834/1/76},
archivePrefix = {arXiv},
       eprint = {1611.04749},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...834...76M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1997rscc.book.....H,
       author = {{Hoyt}, Douglas V. and {Schatten}, Kenneth H.},
        title = "{The role of the sun in climate change}",
         year = 1997,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997rscc.book.....H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1995SoPh..157..389L,
       author = {{Lustig}, G. and {Wohl}, H.},
        title = "{The Growth and Decay of Sunspots: Comparison between the Greenwich and Mount Wilson Sunspot Data}",
      journal = {\solphys},
     keywords = {Decay, Growth, Solar Physics, Sun, Sunspots, Latitude, Umbras, Solar Physics},
         year = 1995,
        month = mar,
       volume = {157},
       number = {1-2},
        pages = {389-392},
          doi = {10.1007/BF00680629},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995SoPh..157..389L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1988A&A...205..289M,
       author = {{Moreno-Insertis}, F. and {Vazquez}, M.},
        title = "{A statistical study of the decay phase of sunspot groups from 1874 to 1939}",
      journal = {\aap},
     keywords = {Photosphere, Statistical Analysis, Sunspots, Decay, Histograms, Magnetic Flux, Solar Physics},
         year = 1988,
        month = oct,
       volume = {205},
       number = {1-2},
        pages = {289-296},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988A&A...205..289M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1993ASPC...46...67M,
       author = {{Martinez Pillet}, V. and {Moreno-Insertis}, F. and {Vazquez}, M.},
        title = "{The Distribution of Sunspot Decay Rates}",
    booktitle = {IAU Colloq. 141: The Magnetic and Velocity Fields of Solar Active Regions},
         year = 1993,
       editor = {{Zirin}, Harold and {Ai}, Guoxiang and {Wang}, Haimin},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {46},
        month = jan,
        pages = {67},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993ASPC...46...67M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993A&A...274..521M,
       author = {{Martinez Pillet}, V. and {Moreno-Insertis}, F. and {Vazquez}, M.},
        title = "{The distribution of sunspot decay rates.}",
      journal = {\aap},
     keywords = {sun: activity, sun: photosphere, sun: sunspots},
         year = 1993,
        month = jul,
       volume = {274},
        pages = {521-533},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993A&A...274..521M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1982SoPh...81...25R,
       author = {{Robinson}, R.~D. and {Boice}, D.~C.},
        title = "{Size Variations in Regular Sunspots}",
      journal = {\solphys},
     keywords = {Periodic Variations, Size Distribution, Sunspots, Astronomical Photography, Magnetic Flux, Solar Physics},
         year = 1982,
        month = nov,
       volume = {81},
       number = {1},
        pages = {25-31},
          doi = {10.1007/BF00151976},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1982SoPh...81...25R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009SoPh..258...13K,
       author = {{Komm}, R. and {Howe}, R. and {Hill}, F.},
        title = "{Emerging and Decaying Magnetic Flux and Subsurface Flows}",
      journal = {\solphys},
     keywords = {Active regions, velocity field, Helioseismology, observations, Interior, convective zone, Velocity fields, interior},
         year = 2009,
        month = aug,
       volume = {258},
       number = {1},
        pages = {13-30},
          doi = {10.1007/s11207-009-9398-6},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009SoPh..258...13K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1967SoPh....1..107G,
       author = {{Gnevyshev}, M.~N.},
        title = "{On the 11-Years Cycle of Solar Activity}",
      journal = {\solphys},
         year = 1967,
        month = jan,
       volume = {1},
       number = {1},
        pages = {107-120},
          doi = {10.1007/BF00150306},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1967SoPh....1..107G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2014SoPh..289..563M,
       author = {{Murak{\"o}zy}, J. and {Baranyi}, T. and {Ludm{\'a}ny}, A.},
        title = "{Sunspot Group Development in High Temporal Resolution}",
      journal = {\solphys},
     keywords = {Sunspots, Solar activity, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = feb,
       volume = {289},
       number = {2},
        pages = {563-577},
          doi = {10.1007/s11207-013-0416-3},
archivePrefix = {arXiv},
       eprint = {1309.1604},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014SoPh..289..563M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...785...90R,
       author = {{Rempel}, M. and {Cheung}, M.~C.~M.},
        title = "{Numerical Simulations of Active Region Scale Flux Emergence: From Spot Formation to Decay}",
      journal = {\apj},
     keywords = {convection, magnetohydrodynamics: MHD, radiative transfer, sunspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = apr,
       volume = {785},
       number = {2},
          eid = {90},
        pages = {90},
          doi = {10.1088/0004-637X/785/2/90},
archivePrefix = {arXiv},
       eprint = {1402.4703},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...785...90R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017ApJ...846..149C,
       author = {{Chen}, Feng and {Rempel}, Matthias and {Fan}, Yuhong},
        title = "{Emergence of Magnetic Flux Generated in a Solar Convective Dynamo. I. The Formation of Sunspots and Active Regions, and The Origin of Their Asymmetries}",
      journal = {\apj},
     keywords = {convection, dynamo, magnetohydrodynamics: MHD, methods: numerical, Sun: magnetic fields, sunspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = sep,
       volume = {846},
       number = {2},
          eid = {149},
        pages = {149},
          doi = {10.3847/1538-4357/aa85a0},
archivePrefix = {arXiv},
       eprint = {1704.05999},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...846..149C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003GeoRL..30.1178C,
       author = {{Chapman}, G.~A. and {Dobias}, J.~J. and {Preminger}, D.~G. and
         {Walton}, S.~R.},
        title = "{On the decay rate of sunspots}",
      journal = {\grl},
     keywords = {Solar Physics, Astrophysics, and Astronomy: Solar irradiance, and Astronomy: Solar and stellar variability, and Astronomy: Stellar interiors and dynamo theory},
         year = 2003,
        month = feb,
       volume = {30},
       number = {4},
          eid = {1178},
        pages = {1178},
          doi = {10.1029/2002GL016225},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003GeoRL..30.1178C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997SoPh..176..249P,
       author = {{Petrovay}, K. and {van Driel-Gesztelyi}, L.},
        title = "{Making Sense of Sunspot Decay. I. Parabolic Decay Law and Gnevyshev-Waldmeier Relation}",
      journal = {\solphys},
     keywords = {Astrophysics},
         year = 1997,
        month = dec,
       volume = {176},
       number = {2},
        pages = {249-266},
          doi = {10.1023/A:1004988123265},
archivePrefix = {arXiv},
       eprint = {astro-ph/9706029},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997SoPh..176..249P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017ApJ...842....3N,
       author = {{Norton}, A.~A. and {Jones}, E.~H. and {Linton}, M.~G. and
         {Leake}, J.~E.},
        title = "{Magnetic Flux Emergence and Decay Rates for Preceder and Follower Sunspots Observed with HMI}",
      journal = {\apj},
     keywords = {Sun: magnetic fields, Sun: photosphere, sunspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jun,
       volume = {842},
       number = {1},
          eid = {3},
        pages = {3},
          doi = {10.3847/1538-4357/aa7052},
archivePrefix = {arXiv},
       eprint = {1705.02053},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...842....3N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...635..659H,
       author = {{Hagenaar}, Hermance J. and {Shine}, Richard A.},
        title = "{Moving Magnetic Features around Sunspots}",
      journal = {\apj},
     keywords = {Sun: Activity, Sun: Magnetic Fields, Sun: Sunspots},
         year = 2005,
        month = dec,
       volume = {635},
       number = {1},
        pages = {659-669},
          doi = {10.1086/497367},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...635..659H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...758..115L,
       author = {{Li}, Jing and {Ulrich}, Roger K.},
        title = "{Long-term Measurements of Sunspot Magnetic Tilt Angles}",
      journal = {\apj},
     keywords = {magnetic fields, Sun: dynamo, Sun: general, Sun: interior, Sun: rotation, sunspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = oct,
       volume = {758},
       number = {2},
          eid = {115},
        pages = {115},
          doi = {10.1088/0004-637X/758/2/115},
archivePrefix = {arXiv},
       eprint = {1209.1642},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...758..115L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1974MNRAS.169...35M,
       author = {{Meyer}, F. and {Schmidt}, H.~U. and {Weiss}, N.~O. and {Wilson}, P.~R.},
        title = "{The growth and decay of sunspots.}",
      journal = {\mnras},
     keywords = {Astronomical Models, Convective Flow, Magnetic Flux, Solar Granulation, Solar Magnetic Field, Sunspots, Decay Rates, Energy Transfer, Evolution (Development), Penumbras, Photosphere, Solar Flux, Time Response, Solar Physics},
         year = 1974,
        month = oct,
       volume = {169},
        pages = {35-57},
          doi = {10.1093/mnras/169.1.35},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1974MNRAS.169...35M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013SoPh..287..215M,
       author = {{McClintock}, B.~H. and {Norton}, A.~A.},
        title = "{Recovering Joy's Law as a Function of Solar Cycle, Hemisphere, and Longitude}",
      journal = {\solphys},
     keywords = {Joy's law, Sunspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = oct,
       volume = {287},
       number = {1-2},
        pages = {215-227},
          doi = {10.1007/s11207-013-0338-0},
archivePrefix = {arXiv},
       eprint = {1305.3205},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013SoPh..287..215M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...758..115L,
       author = {{Li}, Jing and {Ulrich}, Roger K.},
        title = "{Long-term Measurements of Sunspot Magnetic Tilt Angles}",
      journal = {\apj},
     keywords = {magnetic fields, Sun: dynamo, Sun: general, Sun: interior, Sun: rotation, sunspots, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = oct,
       volume = {758},
       number = {2},
          eid = {115},
        pages = {115},
          doi = {10.1088/0004-637X/758/2/115},
archivePrefix = {arXiv},
       eprint = {1209.1642},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...758..115L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





